Doctor AI: Predicting Clinical Events via Recurrent Neural Networks

Leveraging large historical data in electronic health record (EHR), we developed Doctor AI, a generic predictive model that covers observed medical conditions and medication uses. Doctor AI is a temporal model using recurrent neural networks (RNN) and was developed and applied to longitudinal time stamped EHR data from 260K patients over 8 years. Encounter records (e.g. diagnosis codes, medication codes or procedure codes) were input to RNN to predict (all) the diagnosis and medication categories for a subsequent visit. Doctor AI assesses the history of patients to make multilabel predictions (one label for each diagnosis or medication category). Based on separate blind test set evaluation, Doctor AI can perform differential diagnosis with up to 79% recall@30, significantly higher than several baselines. Moreover, we demonstrate great generalizability of Doctor AI by adapting the resulting models from one institution to another without losing substantial accuracy.

==> abst.tex <==
%Large amount of  Electronic Health Record (EHR) data have been collected over millions of patients over multiple years. 
Rich longitudinal Electronic Health Record (EHR)  data documented the collective experiences of physicians including diagnosis, medication prescription and procedures. 
We argue it is possible now to leverage the EHR data to model how physicians behave, and we call our model {\it Doctor AI}. 
{\it Doctor AI} was developed and applied to longitudinal time stamped EHR data on diagnoses and medication and procedure orders from 260K patients over 8 years. We utilized Recurrent Neural Networks (RNN) to jointly forecast all future disease diagnosis categories and medication classes along with their timing. Unlike traditional classification models where a single target is of interest, our model can make continuous and multilabel predictions (i.e., over hundreds of labels for different diagnoses and medications) based on patients' historical data. We evaluate the performance of the proposed method on a large real-world EHR data over 260K patients over 8 years. 
We observed Doctor AI can perform differential diagnosis with similar accuracy to physicians. In particular, Doctor AI achieves up to 79\% recall@30, significantly higher than several baselines. Moreover, we demonstrate  generalizability of Doctor AI by applying the resulting models on data from a different medical institution achieving comparable performance. 

% methods such as logistic regression 31\% and multi-layer perceptron (MLP) 38\%. 
%We further demonstrate that the trained RNNs are capable of transferring information across different hospitals.
%In recent years, large amount of Electronic Health Record (EHR) data have been collected, which allow us to perform sophisticated analysis and solve problems in healthcare that would be considered ambitious years ago.  


==> discuss.tex <==
% \subsection{Assess Prediction Performance %(Table \ref{tab:mainResults})
% }
% %Comparing RNN-based and most frequent past pattern algorithm with the lagged multilayer perceptron algorithm, we postulate that the status of the patients in this dataset depends on more than 5 lags.
% The superior performance of RNN based approaches can be attributed to the efficient representation that they learn for patients at each visit \citep{bengio2013representation,schmidhuber2015deep}. RNNs are able to learn succinct feature representations of patients by accumulating the relevant information from their history and the current set of codes, which outperformed ad hoc feature engineering.
% %Given our network structure and the loss function, we can observe from the experimental results that the hidden layer of the RNN significantly out-performs at learning efficient representations for the patient status than ad-hoc feature engineering (\textit{e.g.} \textit{tf-idf} features used in the baseline models) such that a simple linear classifier can effectively predict the codes of the next visit.

% %The results also suggest that increasing the number of lags in the logistic and MLP approaches may not significantly improve the performance.  Given the size of the dataset, this can be due to overparameterization of the model that may push the models to the boundary of high-dimensionality. While we use $L_1$ regularization in both cases, the result indicates that it cannot fully prevent noise accumulation due to noisy input dimensions.

% Table \ref{tab:mainResults} confirms that learning patient representation with RNN is easier with the input vectors that are already efficient representations of the medical codes. The RNN trained with the Skip-gram vectors (denoted by RNN-IR) consistently outperforms the RNN that learns the weight matrix $\Wb_{emb}$ directly from the data, with only one exception, the medication prediction Recall@30, although the differences are insignificant. The results also confirm that having multiple layers when using RNN improves its ability to learn more efficient representations. The results also indicate that a single layer RNN might have enough representative power to capture the dynamics of medications, and adding more layers may not improve the performance.

% The results also indicate that our approach significantly improves the accuracy of predicting the time duration until the next visit compared to the baselines. However, the absolute value of $R^2$ metric shows that accurate prediction of time intervals remains as a challenge. We believe achieving significantly better time prediction without extra features should be difficult because the timing of a clinical visit can be affected by many personal factors such as financial status, location of residence, means of transportation, and life style, to name a few. Thus, without such sensitive personal information, which is rarely included in the EHR, accurate prediction of time intervals should be unlikely.

% \noindent \textbf{Discussion for Figure \ref{fig:overTime}}
% We believe that the increase in performance can be due to two reasons: (1) RNN is able to learn a better estimate of the patient status as it sees longer patient records and (2) the patient's status stabilizes over time and the prediction task becomes easier.

% \noindent \textbf{Discussion for Figure \ref{fig:perplexity}}
% Figure \ref{fig:perplexity} shows contrasting patterns: when the input is one of the frequent codes such as hypertension, the network quickly learns a more specific set of output codes as next disease. When we select an infrequent code like Klinefelter's syndrome as the input, the network's output is more diverse and mostly the frequently observed codes. The top 30 codes after convergence shown in Table \ref{tab:visu} in Appendix \ref{sec:qual} confirm the disparity of the diversity of the predicted codes for the two cases.
To take a closer look at the performance of Doctor AI, in Table \ref{tab:qual} (in Appendix \ref{sec:qual}) we list the predicted, true, and historical diagnosis codes for five visits of different patients. The blue items represent the correct predictions. The results are promising and show that, given the history of the patient, the Doctor AI can predict the true diagnostic codes. The results highly mimic the way a human doctor will interpret the disease predictions from the history. For all five of the cases shown in Table \ref{tab:qual}, the set of predicted diseases contain most, if not all of the true diseases. For example, in the first case, the top 3 predicted diseases match the true diseases. A human doctor would likely predict similar diseases to the ones predicted with Doctor AI, since old myocardial infarction and chronic ischemic heart disease can be associated with infections and diabetes \citep{stevens1978diabetic}.

In the fourth case, visual disturbances can be associated with migraines and essential hypertension \citep{keith1939some}. Further, essential hypertension may be linked to cognitive function \citep{kuusisto1993essential}, which plays a role in anxiety disorders and dissociative and somatoform disorders. Regarding codes that are guessed incorrectly with the fourth case, they can still be plausible given the history. For example, cataracts, and disorders of refraction and accommodation could have been guessed based on a history of visual disturbances, as well as strabismus and disorders of binocular eye movements. Allergic rhinitis could have been guessed, because there was a history of allergic rhinitis. In summary, Doctor AI is able to very accurately predict the true diagnoses in the sample patients. The results are promising and should motivate future studies involving the application of Doctor AI on different datasets exhibiting other populations of patients.


% \paragraph*{Interpretability}
%In healthcare, it is desirable to have models that are interpretable; i.e., models' parameters can be translated to clinically meaningful quantities that physicians or patients understand. However, there is a well-known trade-off between interpretability (intelligibleness) and accuracy of machine learning algorithms \cite{caruana2015intelligible}. Neural networks, and in particular Recurrent Neural Networks, are more on the accurate side rather than the intelligible side  of the trade-off spectrum. Although, several recent attempts have been made to interpret the parameters of RNNs, such as \cite{ghosh1992sequence} and this problem remains an active line of research \cite{karpathy2015visualizing,che2015distilling}. Interpretability can be considered a limitation of RNN in healthcare applications, although we believe the significant gain in accuracy in this approach outweighs the limitation. 

%While interpretability of the model is desirable in healthcare applications, the accurate black-box models can still be useful. In fact, the common clinical practice does not require practitioners to fully understand the underlying mechanism of how a particular drug or lab test works. For example, pharmaceutical companies are not required to show exactly why their proposed medicine works. They only need to show efficacy through randomized control trials. In the same spirit, with this early evidence from this work, Doctor AI can be prospectively validated through randomized clinical trials in order to apply in practice. %\ecedit{What do you mean by "with this early evidence from this work"?}

%Finally, it is worth mentioning that interpretability of machine learning algorithms usually requires a discussion about causality and whether the algorithm can uncover causal relationships. Despite the fact that most of the common machine learning algorithms are not guaranteed to find causal relationships between features and labels, we still find them useful, because they provide \textit{accurate prediction} of the target label \cite{spirtes2010introduction}. Similarly, Doctor AI's main objective is to provide accurate diagnostic and medication prediction which can be of great value in practice as a clinical decision support tool.

==> introNew.tex <==
The broad adoption of Electronic Health Records (EHR) has continuously generated large amount of patient data that documents rich clinical interactions over time. 
This high-dimensional longitudinal data has created an opportunity to perform sophisticated temporal analysis that was not possible before. 
Forecasting clinical events for patients is an especially challenging, yet important task. Our goal is to develop a temporal prediction model that mimics physician practice based on the collective memory of many physicians, i.e., large amount of EHR data over a long period of time.
%that attempts to predict occurrence of various diseases over time for individual patients and what type of actions will be taken by the physicians.
Successfully forecasting clinical events can not only facilitate patient-specific care and timely intervention, but also potentially reduce healthcare cost.% for those who are not allowed easy access to clinical facilities.}
%\sout{Successful forecasting will facilitate patient-specific care and timely intervention, thus reducing overwhelming health care costs and saving human lives.}

Although related problems such as disease progression modeling have been studied by many researchers over several decades, e.g. \cite{Heckerman:1990,chapman2001simple,lange2015joint}, most works do not achieve required accuracy and scalability, or need excessive expert domain knowledge, partly due to the lack of rich longitudinal EHR data and scalable computational architecture.
Thanks to the recent advances in recurrent neural network, we propose \textit{Doctor AI} system that can diagnose multiple disease conditions and prescribe relevant medications based on historical EHR data. 
Furthermore, the Doctor AI tries to predict when the patient will make the next visit. Our ultimate goal is to have Doctor AI help both health providers and patients. 

\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{./Figs/DoctorAI}
\caption{Doctor AI extracts clinical events as multilable point process data from EHR and learns a model for patient status dynamics.  Given a new patient's record, it can forecast the patient's diagnoses (Dx), prescribed medications (Rx), and the time until his/her next visit. }
\end{figure}

The problem in general can be described as a multilabel marked point process modeling task.
The task is different from common sequential learning tasks such as those in natural language processing as it requires prediction of multiple categories over the continuous time axis.
The key challenge in this task is to find a flexible model that is capable of predicting multiple event types for patients. 
The two main classes of techniques, continuous-time Markov chain based models \cite{nodelman2002continuous,lange2015joint,johnson2013bayesian}, and intensity based point process modeling techniques such as Hawkes processes \cite{liniger2009multivariate,zhu2013nonlinear,choiconstructing2015} have been proposed but they are expensive to generalize to nonlinear and multilabel settings.
Furthermore, they often make strong assumptions about the data generation process which might not be valid in large-scale EHR datasets.

The key idea of this paper is to learn an effective representation of the patient status over time and to leverage such representation to predict future clinical events of the patients such as diagnoses and medication prescriptions and their timings.  
To learn such patient representations we propose to use recurrent neural networks (RNN), considering the fact that patients have different length of medical records and that recurrent neural networks have been shown to be particularly successful for representation learning in sequential data, \textit{e.g.} \cite{graves2013generating,graves2014towards,sutskever2014sequence,kiros2014unifying,zaremba2014learning}.
In particular, we make the following main contributions in this paper:
\begin{itemize}
\item We demonstrate a successful application of RNNs in representing the status of patients, predicting the future clinical events and the timing of the events. The trained RNN is able to achieve above 64\% (79\%) recall in its top 10 (30) predicted diagnosis codes, demonstrating great potential as a computerized differential diagnosis guide. 
\item We propose an efficient initialization scheme for RNNs using Skip-gram embedding \cite{mikolov2013distributed} and show that it improves the performance of the RNN in both accuracy and speed.
\item We empirically confirm that RNNs can be used to transfer knowledge across multiple medical institutions. This suggests that hospitals with insufficient patient records can adopt the models learned from larger data of other health institutions to improve the quality of their clinical service.
\end{itemize}


==> oldResultTable.tex <==
% \begin{table}[ht]   
% \centering
% \caption{Accuracy of algorithms in forecasting the future medical activities.}
% \label{tab:mainResults}
% {\renewcommand{\arraystretch}{1.1}
% \begin{tabular}{l|c|c|c|c}
%  & \multicolumn{3}{c|}{Percentage Recall @$k$} &\% $R^2$\\
% Algorithms & $k=10$& $k=20$&$k=30$ & $\log(\Delta t)$\\
% \hline
% \hline
% Previous visit's codes & \multicolumn{3}{|c|}{26.25} & -- \\
% Most frequent past codes & 48.11 & 60.23 & 66.00 & -- \\
% Logistic &17.66 & 26.12 & 31.23& 0.0013 \\
% MLP & 19.49& 30.80& 38.13& 0.0017\\
% Hawkes  & & & & \\
% \hline
% RNN-1 (Dx) & 63.12 & 73.11 & 78.49 & e20 \\
% RNN-2 (Dx) & 63.32 & 73.32 & 78.71 & e20 \\
% %RNN-3 (Dx) & 60.96 & 70.99 & 76.59 & e20,h1000\\
% \hline 
% RNN-1-IR (Dx) & 63.24 & 73.33 & 78.73 & e20 \\
% RNN-2-IR (Dx) & 64.30 & 74.31 & 79.58 & e20 \\
% %RNN-3-IR (Dx) & 64.07 & 74.08 & 79.40 & e20 \\
% \hline
% RNN-1 (Rx) & & & & \\
% RNN-2 (Rx) & & & & \\
% \hline
% RNN-1-IR (Rx) & & & & \\
% RNN-2-IR (Rx) & & & & \\
% \hline
% RNN-1 (Time) & & & & \\
% RNN-2 (Time) & & & & \\
% \hline
% RNN-1-IR (Time) & & & & 0.2539, e20 \\
% RNN-2-IR (Time) & & & & \\
% \hline
% RNN-1 (Dx,Rx,Time) & 53.86 & 65.10 & 71.24 & 0.2519, e20 \\
% RNN-2 (Dx,Rx,Time) & 53.61 & 64.93 & 71.14 & 0.2528 \\
% %RNN-3 (Dx,Rx,Time) & & & & \\
% \hline
% RNN-1-IR (Dx,Rx,Time) & 54.37 & 65.68 & 71.85 & 0.2492, e20 \\
% RNN-2-IR (Dx,Rx,Time) & 54.96 & 66.31 & 72.48 & 0.2534, e20 \\
% %RNN-3-IR (Dx,Rx,Time) & & & & \\
% \hline
% \end{tabular}
% }
% \end{table}


\begin{table}[t]   
\centering
% \begin{center}
\caption{Accuracy of algorithms in forecasting future medical activities.}
\label{tab:mainResults}
{\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}l@{\;}||@{\;\;}c@{\;}|@{\;}c@{\;}|@{\;}c@{\;\;}||@{\;}c@{\;}|@{\;}c@{\;}|@{\;}c||@{\;}c@{\;}|@{\;}c@{\;}|@{\;}c@{\;}|@{\;\;}c@{}}
 & \multicolumn{3}{@{\;}c@{\;}||@{\;}}{Dx Only Recall @$k$} & \multicolumn{3}{@{\;}c@{\;}||@{\;}}{Rx Only Recall @$k$} & \multicolumn{4}{c}{Dx,Rx,Time Recall @$k$}\\
Algorithms & $k=10$& $k=20$&$k=30$ & $k=10$& $k=20$&$k=30$ & $k=10$& $k=20$&$k=30$& $R^2$ \\
\hline
\hline
Last visit & \multicolumn{3}{@{\;}c@{\;}||@{\;}}{29.17} & \multicolumn{3}{@{\;}c@{\;}||@{\;}}{13.81} &\multicolumn{3}{c}{26.25}& ---\\
Most freq.  &56.63 &67.39 &71.68 & 62.99 &69.02 &70.07 & 48.11 & 60.23 & 66.00& --- \\
Logistic (L=1) &22.97 &32.20 &36.58 &28.01 &39.75 &43.79 &17.66 & 26.12 & 31.23 & 0.0013 \\
MLP (L=1) &26.09 &39.19 &48.04 &32.27 &51.12 &61.50 & 19.49& 30.80& 38.13& 0.0017 \\
Logistic (L=5)  & 26.04&39.17 &48.19 &32.39 &51.06 &61.03 &18.79 &29.13 & 35.63&0.0013 \\
MLP (L=5)  &26.14 &39.41 &48.28 &32.39 & 51.18& 61.66 &19.32 &30.77 &38.08 & 0.0002\\
Feature Ext. &26.12 &39.33 &48.20 &32.27 &51.12 &61.65 &19.60 & 30.80 & 38.13 & 0.0022\\
%Hawkes  & & & & & & & & & & ---\\
\hline
RNN-1 & 63.12 & 73.11 & 78.49 & 67.99 & 79.55 & \textbf{85.53} & 53.86 & 65.10 & 71.24 & 0.2519\\
RNN-2 & 63.32 & 73.32 & 78.71 & 67.87 & 79.47 & 85.43 & 53.61 & 64.93 & 71.14 & 0.2528\\
\hline
RNN-1-IR & 63.24 & 73.33 & 78.73 & \textbf{68.31} & \textbf{79.77} & 85.52 & 54.37 & 65.68 & 71.85 & 0.2492 \\
%RNN-1-IR (d1000) & & & & & & & & & & \\
RNN-2-IR & \textbf{64.30} & \textbf{74.31} & \textbf{79.58} & 68.16 & 79.74 & 85.48 & \textbf{54.96} & \textbf{66.31} & \textbf{72.48} & \textbf{0.2534}\\
\hline
\end{tabular}
}
\end{table}
% 18.46 &27.55 & 32.71  for logistic all
